NeuSpeech: Decode Neural signal as Speech

Decoding language from brain dynamics is an important open direction in the realm of brain-computer interface (BCI), especially considering the rapid growth of large language models. Compared to invasive-based signals which require electrode implantation surgery, non-invasive neural signals (e.g. EEG, MEG) have attracted increasing attention considering their safety and generality. However, the exploration is not adequate in three aspects: 1) previous methods mainly focus on EEG but none of the previous works address this problem on MEG with better signal quality; 2) prior works have predominantly used $``teacher-forcing"$ during generative decoding, which is impractical; 3) prior works are mostly $``BART-based"$ not fully auto-regressive, which performs better in other sequence tasks. In this paper, we explore the brain-to-text translation of MEG signals in a speech-decoding formation. Here we are the first to investigate a cross-attention-based ``whisper" model for generating text directly from MEG signals without teacher forcing. Our model achieves impressive BLEU-1 scores of 60.30 and 52.89 without pretraining $\&$ teacher-forcing on two major datasets ($\textit{GWilliams}$ and $\textit{Schoffelen}$). This paper conducts a comprehensive review to understand how speech decoding formation performs on the neural decoding tasks, including pretraining initialization, training $\&$ evaluation set splitting, augmentation, and scaling law. Code is available at https://github.com/NeuSpeech/NeuSpeech1$.

==> text/table_target_abl_splits.tex <==
\begin{wraptable}{l}{0.5\textwidth}
    \centering
    \caption{Transcription results on different splits, where \textbf{bold} denotes a correct match between ground truth and our prediction. \underline{Underline} denotes a fuzzy match with similar semantic meanings.} 
    
    %Performance on word-level EEG features is significantly better as the task is easier. Still, decoding on raw waves could output meaningful results.
    \label{tab:generation_results_splits} 
    
    \footnotesize
    % \setlength{\tabcolsep}{1.9pt}
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{p{8cm}}
    % \begin{tabular}{}
         
     \toprule 
     
     \textbf{Hold-out sentences}\\ \midrule
     
     Ground Truth: I looked down and saw he was pointing to another marker just slightly \underline{\textbf{different} from the one we had just left} \\
     % \hline
     Prediction: \underline{It was \textbf{different} from now} and it just wasn't working well. \\\midrule
     \textbf{Hold-out story}\\ \midrule
     
     Ground Truth: Mahogany \textbf{black} curly hair cut short in the typical military style framed a dark skinned face \\
     % \hline
     Prediction: I must admit, this is a great \textbf{black} or cold weather. It had things such as 
    \\\bottomrule
    \end{tabular}
% \vspace{-15pt}
    }
\end{wraptable}
% \colorbox{orange}{\underline{deaths}} 
